Lattice QCD study of the elastic and transition form factors of charmed baryons

I review the progress made in calculating the elastic and transition form factors of charmed baryons from lattice simulations.

==> em/diag/secs/mesonff.tex <==
Parameterization of an interaction in terms of form factors depends on the spin of the hadron in question. For a \spinze meson, $\mcm$, the electromagnetic interaction matrix element is parameterized by a single form factor,
\begin{align}\label{eq:s0_me}
	\langle \mcm(\pp)| \mathcal{V}_\mu(q) | \mcm(p) \rangle = (p + \pp)_\mu F_\mcm(Q^2),
\end{align}
whereas for a \spinon meson, $\mcms$, there are three form factors~\cite{Brodsky:1992px},
\begin{align}\label{eq:s1_me}
	\begin{split}
		\langle \mcms(\pp,\ssp)| \mathcal{V}_\mu(q) | \mcms(p,s) \rangle &= \epsilon^{\prime \ast}_\tau(\pp, \ssp)
		\left\{ g^{\tau\sigma} (p + \pp)_\mu \tilde{G}_1(Q^2) \right. \\
		&\left.- (g_\mu{}^\tau q^\sigma - g_\mu{}^{\sigma} q^\tau) \tilde{G}_2(Q^2) \right. \\
		&\left.- (p + \pp)_\mu \frac{q^\tau q^\sigma}{2 m^2_{\ast}} \tilde{G}_3(Q^2) \right\} \epsilon_\sigma(p,s).
	\end{split}
\end{align}
Here, $\epsilon$ and $\epsilon^\prime$ are the polarization vectors, $p$ and $\pp$ are the four-momenta, and $s$ and $\ssp$ are the spin of the initial and final states, respectively. $m_\ast \equiv m_\mcms$, is the mass of the \spinon meson. We use the notation, $Q^2 = -q^2 = -(p-\pp)^2$. The form factors $\tilde{G}_{i}$ are arranged in terms of Sachs electric, magnetic and quadrupole form factors as follows~\cite{Brodsky:1992px,Arnold:1980zj},
\begin{align}\label{eq:s1_sachs}
	F_C(Q^2) &= \tilde{G}_1(Q^2) + \frac{2}{3}\tau F_Q(Q^2), \\
	F_M(Q^2) &= \tilde{G}_2(Q^2), \\
	F_Q(Q^2) &= \tilde{G}_1(Q^2) - \tilde{G}_2(Q^2) + (1+\tau) \tilde{G}_3(Q^2),
\end{align}
where $\tau = Q^2/4m^2_\ast$.

==> em/diag/secs/tables/ddrho_res.tex <==
%%%%%%%%% Table of DDrho results %%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\tbl{The coupling constants $g_{DD\rho}$, $g_{D^\ast D^\ast\rho}$ obtained from VMD fits and the charge radius of D and D$^\ast$ mesons obtained from monopole fits together with the individual quark-sector contributions. The extrapolated results are from linear and quadratic fits discussed in the main text. }
	{
	\begin{tabular}{@{}ccccc@{}} \toprule
		\texttt{ID}   & $g_{DD\rho}$  &  $\langle r_{D}^2 \rangle$ (fm$^2$) & $\langle r_{D,d}^2 \rangle$ (fm$^2$) & $\langle r_{D,c}^2 \rangle$ (fm$^2$) \\
		\colrule
		\ensh     & 5.57(27) & 0.098(8)\pz & 0.226(20)\pz & 0.040(9)\pz \\
		\enh      & 5.03(28) & 0.094(10)   & 0.232(29)\pz & 0.033(9)\pz \\
		\enm      & 5.30(30) & 0.124(13)   & 0.350(50)\pz & 0.033(12)   \\
		\enl      & 4.85(41) & 0.133(19)   & 0.308(85)\pz & 0.059(13)   \\
		Lin. Fit  & 4.84(34) & 0.138(13)   & 0.342(67)\pz & 0.051(11)   \\
		Quad. Fit & 4.90(56) & 0.152(26)   & 0.320(118)   & 0.074(16)   \\ 
		\colrule
		% 
		\texttt{ID}   & $g_{D^*D^*\rho}$  &  $\langle r_{D^\ast}^2 \rangle$ (fm$^2$) & $\langle r_{D^\ast,d}^2 \rangle$ (fm$^2$) & $\langle r_{D^*,c}^2 \rangle$ (fm$^2$) \\
		\colrule
		\ensh     & 5.93(41) & 0.106(12) & 0.270(31)\pz & 0.035(13) \\
		\enh      & 5.75(36) & 0.113(17) & 0.296(44)\pz & 0.036(14) \\
		\enm      & 6.69(47) & 0.167(25) & 0.497(92)\pz & 0.044(21) \\
		\enl      & 5.57(66) & 0.169(30) & 0.404(127)   & 0.075(26) \\
		Lin. Fit  & 5.94(56) & 0.185(24) & 0.475(94)\pz & 0.071(16) \\
		Quad. Fit & 5.42(94) & 0.192(43) & 0.406(156)   & 0.096(29) \\ \botrule
	\end{tabular} \label{tab:ddrho_res}
	}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

==> mass/secs/ground.tex <==
Once the two-point correlation function is computed on the quark level, it is theoretically a simple procedure to extract the mass of the hadron via use of \Cref{eq:2pt_fit}. In practice, however, it is a matter of identifying a reliable signal region. The two-point correlation function contains not only the ground state of the hadron but also all the possible excited states or multi-quark states that correspond to the same quantum numbers as given in \Cref{eq:2pt_sum_simp}. Only in the large Euclidean-time limit the ground state dominates. The standard technique to identify from which time slice the ground state dominates is to investigate a quantity called the \emph{effective mass},  
\begin{equation}
	\label{eq:effmass}
	m_{\rm eff}(t) = \frac{1}{\Delta t} \operatorname{ln} \frac{\mathcal{G}(t)}{\mathcal{G}(t + \Delta t)},
\end{equation} 
which forms a plateau with respect to evolving time at sufficiently large time slices before the signal is lost to statistical noise. The plateau region is then identified as the ground state and its energy is extracted from the two-point correlation function by a nonlinear regression of choice with \Cref{eq:2pt_fit} being the model function. 

Any systematical uncertainty related to the excited state contamination can be taken into account by modeling the excited states as additional exponential terms,
\begin{equation}
	\langle \mathcal{G}(t; {\bf p}; \Gamma) \rangle =  A_0 e^{-E_0({\bf p}) t} \left( 1 + \sum_{n=1} A_n^\prime e^{-\Delta E_n({\bf p}) t} \right),
\end{equation}
where $E_0$ is the energy of the ground state, $A_n^\prime = A_n/A_0$, and $\Delta E_n({\bf p}) = E_n({\bf p}) - E_0({\bf p})$ is the energy gap between the ground state and the n$^{\rm th}$ excited state.    

==> mass/secs/mass.tex <==
Mass plots results
